Timely Detection and Mitigation of Stealthy DDoS Attacks via IoT Networks

Internet of Things (IoT) networks consist of sensors, actuators, mobile and wearable devices that can connect to the Internet. With billions of such devices already in the market which have significant vulnerabilities, there is a dangerous threat to the Internet services and also some cyber-physical systems that are also connected to the Internet. Specifically, due to their existing vulnerabilities IoT devices are susceptible to being compromised and being part of a new type of stealthy Distributed Denial of Service (DDoS) attack, called Mongolian DDoS, which is characterized by its widely distributed nature and small attack size from each source. This study proposes a novel anomaly-based Intrusion Detection System (IDS) that is capable of timely detecting and mitigating this emerging type of DDoS attacks. The proposed IDS's capability of detecting and mitigating stealthy DDoS attacks with even very low attack size per source is demonstrated through numerical and testbed experiments.

==> odit__2_.tex <==
\section{Proposed Anomaly-Based IDS }
\subsection{Online Discrepancy Test}
\label{s:algorithm}
The dynamic nature of an IoT network makes parametric anomaly detection approaches to detect a DDoS attack less effective since they assume probabilistic models for nominal and anomalous conditions. On the other hand in practice it is difficult to know the anomalous distribution. Hence, parametric anomaly based IDSs, as well as many conventional signature-based IDSs are not feasible. Recently, an online and non-parametric detector called the Online Discrepancy Test (ODIT) was proposed for detecting persistent and abrupt anomalies. Thanks to its nonparametric operation, ODIT does not need to know baseline or anomalous distributions/patterns beforehand, hence can address the challenge (C2) stated in Section I \cite{ODIT}. ODIT is a sequential method which accumulates evidence in time, and makes a decision at each time based on the accumulated evidence so far,  instead of making a hard decision based on a single data point. That sequential nature of ODIT is tailored for timely detection, thus it is able to address the challenge (C3). Moreover, ODIT can handle monitoring large number of devices together (see Section IV), which addresses the challenge (C1). 

\begin{figure}[t]
\centering
\includegraphics[width=.35\textwidth]{graph.pdf}
\caption{ODIT procedure with $N_1=5$, $N_2=10$, $M=4$, $k=2$, $s=1$, $\gamma=1$. $L_1-L_{(M)}$ and $L_2-L_{(M)}$ are used as in \eqref{e:Dt} for online anomaly detection (see also Fig. \ref{f:odit}). Test points are from the same nominal distribution as training points, which is a two-dimensional Gaussian with independent components with $0.5$ mean and $0.1$ standard deviation.}
\label{f:graph}
\end{figure}

The Cumulative Sum (CUSUM) is the optimum sequential change detection algorithm, in the minimax sense, under the assumption that both the nominal distribution and the anomalous distribution are completely known. Due to the unknown attack strategies (i.e., attacked devices, and attack magnitudes), it is unrealistic to assume that the anomalous distribution would be known. The practical version of CUSUM, which is called generalized CUSUM assumes parametric distributions for the nominal and anomalous distributions (e.g., $f_0$ and $f_1$), and estimates their parameters from data. However, it is even difficult to select a good baseline model $f_0$, as a brief study of the data genearated by the IoT devices show that they often include short bursts of data packets. Hence, a nonparametric detector, such as the Geometric Entropy Minimization (GEM) algorithm, suits better to attack detection in IoT networks than the parametric detectors. GEM is also computationally efficient such that it scales well to high dimensional problems \cite{Hero}. Nevertheless, GEM decides based on a single observation at each time (i.e., non-sequential), and thus lacks the timely detection capability of CUSUM. The reason why ODIT well addresses the challenges (B1)-(B3) for IoT network security is the fact that ODIT successfully combines the nonparametric and computationally efficient nature of GEM with the sequential operation of CUSUM. 

We next show the procedure for the proposed ODIT-based IDS for node  (see Fig. \ref{no_anomaly}), which observes the $D$-dimensional normalized data vector $x_t^k \in [0,1]^D$, where $D$ is the number of devices, at each time $t$. Here, in the context of DDoS attack detection, $x_t^k$ denotes the number of packets received from the $D$ devices in the network at time $t$ and normalized by the corresponding maximum number of packets for each device. We start with the training procedure:
\begin{enumerate}

\item Acquire an attack training dataset $\mathcal{X}_N=\{\mathcal{x}^{j}_1,\ldots,\mathcal{x}^{j}_N\}$ which represents the baseline (i.e., nominal) operation. Randomly separate it into two subsets $\mathcal{X}^{N_1}$ and $\mathcal{X}^{N_2}$ for computational efficiency, as in the bipartite GEM algorithm\cite{Bass}. 
\vspace{5mm}
\item For each point in $\mathcal{X}^{N_1}$ find the $k$ nearest neighbors from $\mathcal{X}^{N_2}$ , and forms an $M$-point $k$-nearest-neighbor ($M$-$k$NN) Euclidean graph $G=(\mathcal{X}^{N_1}_M,E)$ by selecting the $M$ points $\mathcal{X}^{N_1}_M$ in $\mathcal{X}^{N_1}$ with the smallest total edge length and their $k$ closest neighbors in $\mathcal{X}^{N_2}$, where $E=\{e_{m(n)}\}$ is the set of edges with $e_{m(n)}$ denoting the edge between point $m$ in $\mathcal{X}^{N_1}$ and its $n$th nearest neighbor in $\mathcal{X}^{N_2}$. 
The total edge length of a point $m$ in $\mathcal{X}^{N_1}$ is given by
\begin{equation}
\label{e:length}
L_m = \sum_{n=k-s+1}^k |e_{m(n)}|^\gamma,
\end{equation}
\end{enumerate}
\vspace{5mm}



After training, whenever a new data $x_t^k$ is observed at time $t$:
\begin{enumerate}
\item Compute the statistic as
\vspace{5mm}
\begin{equation}
\label{e:Dt}
D_t = L_t - L_{(M)}
\end{equation} 

where $L_t$ is the total edge length of the new data point $x_t^k$ with respect to the points in $\mathcal{X}^{N_2}$, and $L_{(M)}$ is the total edge length of the $M$th (i.e., boundary) point in the graph $\mathcal{X}_M^{N_1}$ obtained in the training. /cite{Bass}


\vspace{5mm}
\item Treating the statistic $D_t$ as a positive/negative evidence for anomaly accumulate it over time as in CUSUM:
\begin{equation}
s_t^k = \max\{s_{t-1}^k + D_t,0\}, s_0^k=0,
\end{equation}
\end{enumerate}

where $D_t$ is given in \eqref{e:Dt}. At each time $t$, ODIT decides to continue taking a new data point $x_{t+1}^k$ if the accumulated evidence $s_t^k$ is not sufficient for raising an attack alarm. In other words, ODIT stops the first time $s_t^k \ge h$, i.e., 
\begin{equation}
T_k = \min\{t: s_t^k \ge h\},
\end{equation}
$h>0$ is a predetermined threshold, and raises an alarm. The detection threshold $h$ manifests a trade-off between minimizing the detection delay and minimizing the false alarm rate, as can be seen in Fig. 5. Particularly, smaller threshold facilitates early detection, but also increases the probability of false alarm. In practice, $h$ can be chosen to satisfy a given false alarm rate.

\vspace{5mm}
For the ODIT-based IDS, the training and the computation of statistic at each time is illustrated in Fig. 4, and a realization of the accumulated test statistic $s_t$k is given in Fig. 5.

\begin{figure}[t]
\centering
\includegraphics[width=.37\textwidth]{odit_stat1.pdf}
\caption{ODIT statistic and decision procedure using the setup in Fig. \ref{f:graph} and anomalous test points from uniform distribution over $[0,1]$. Anomaly starts at $t=6$, and detected at $t=7$ with the shown threshold.}
\label{f:odit}
\end{figure}

Using the proposed local IDS for each node $k$, it is possible to develop a distributed global IDS by collecting the local decision statistics $\{s_t^k\}_k$. Hence, we also propose a system-wide detector in which each node $k$ does not decide alone based on its data $\{\vx^{k}_t\}$, but instead cooperates with other nodes by passing its test statistic $s^{k}_t$ to the center. 

\subsection{Mitigation Strategy}

Quickest detection of a DDoS attack via an IoT network is a neccessary but not a sufficient condition for ensuring the security of a system. We need a Mitigation Strategy that should be capable of stopping the DDoS attack by locating the anomalous IoT devices connected to it and then employing a strategy such as dropping the packets originating from the pacticular IoT device. The ability to find the source of an IP packet without relying on the source IP field in the packet, which might be spoofed, is called IP traceback analysis. 

We perform an in-depth analysis by examining every dimension, which represent an IoT device connected to the node, of the statistic calculated in Section III-A and computing which IoT device is causing the increase. We next show the procedure for the proposed Mitigation Strategy, which observes the $D$-dimensional data vector $x_t D$, where $D$ is the number of devices, at each time $t$.

 Previously, in the proposed IDS we computed the statistic $L_t$, which was the total edge length of the new data point $x_t^D$ with respect to the points in $\mathcal{X}^{N_2}$. In this section, we further analyze $L_t$ as a $D$-dimensional data vector $r_d$, where each dimension corresponds to the euclidiean distance between the new data point belonging to the particular dimension with respect to the points in $\mathcal{X}^{N_2}$. Based on this, we compute the statistic $\overline{r_d}$,


where $\overline{r_d}$  =  $1/T$ ($\sum\limits_{t=\tau}^{T+\tau} r_td$)





==> simulation_results.tex <==
\subsection{Simulation Results}
The simulation setup consists of $100$ devices connected to a single node (Fig. \ref{f:odit}); and a cooperative setup with $10$ nodes each of which monitor $100$ devices (Fig. \ref{f:odit-mult}) . The IoT devices considered here are those that are most likely to be compromised or devices that are present in every smart home. The devices are assumed to have two states of operation, idle state and active state. The assumed probabilities of the devices being in idle or active state is given by Table \ref{table:2}. The setup of DoS/DDoS simulations is shown in Fig. \ref{f:anomaly}, in which we inject the attack traffic of different rates into the simulated dataset and apply the proposed detection and mitigation scheme to diagnose these attacks. We perform this repeatedly for different kinds of scenarios in which various combinations of devices get attacked to compute the Average Detection Delay vs. False Alarm Rate (i.e., false alarm probability) performance. Now let us take a look at the data model and attack model assumed for the simulations.

\textbf{\textit{Data Model:}} In each node, we assume data from IoT devices are independent and identically distributed (iid) following the pattern given in Table \ref{table:2}. The probabilities listed are based on heuristics and standard day-to-day usage of the mentioned devices. For example, a smart TV is considered to be used approximately 7 to 8 hours in a day, so its active state probability is given as 0.3. 
With the shown probabilities devices may or may not switch state after a session. We consider the following session durations: $5$ sec. for thermostat, $10$ sec. for smart light, $40$ sec. for smart printer, $900$ sec. for smart TV, and ``always on" for security camera.
The mean packet rates are determined by considering the amount of data that is transmitted per second and the average packet size. 
%\tb{
For each device, the number of packets are generated using the mixture of two Gaussian distributions defined by the active state probability, mean packet rates and a common standard deviation, chosen as $5$. To obtain the number of packets the generated real-valued numbers are rounded to the nearest nonnegative integer.
%}
For the purpose of simulation, the training data consists of 40 hours of attack-free data from 100 different devices. 

\textbf{\textit{Attack Model:}} Here we consider a practical scenario in which the IoT devices could be under attack, but the node is assumed to be secure. To parameterize the attack size, we consider 10\% of the devices to be compromised. The attacked devices are randomly selected to assume a general model. During the attack phase, the data rates of the selected devices are increased slightly by 20\%. 

%\tb{
\textbf{\textit{Comparisons:}} We compare our proposed model with CUSUM, which knows the exact parameters of the nominal model and the anomalous model, as well as with Generalized CUSUM (G-CUSUM), which estimates the parameters of the nominal and anomalous Gaussian models from training data.  Note that G-CUSUM uses training data for the attack scenarios, as opposed to ODIT, which is blind to the attack scenarios. 
CUSUM knows exactly the mean and standard deviation of the Gaussian distribution, as well as the probability of being active for each device. Note that due to rounding to the nearest nonnegative integer value, the real probability distribution of number of packets deviates from the generative bimodal Gaussian.  %On the other hand, to show the effect of errors in estimating the parameters we also compare with CUSUM inflicted by $5\%$ error in both mean and standard deviation estimation.
Hence, the proposed ODIT detector even sometimes outperforms CUSUM, which exactly knows the generative Gaussian model. The results for Average Detection Delay vs False Positive Rate (i.e., false alarm probability) are shown in Fig. \ref{f:odit} and Fig. \ref{f:odit-mult}. We see that the proposed IDS performs closely to the clairvoyant CUSUM detector which exactly knows the generative probabilistic model, and significantly outperforms the other practical detectors, namely G-CUSUM, the data filtering method, and the information metric method proposed in \cite{Informetric}. The filtering method is a straightforward detector which simply applies a threshold to the observed raw data, i.e., declares an alarm if the data rate of a device exceeds the threshold. The information metric method proposed in \cite{Informetric} uses an information distance metric based on the generalized (R{\'e}nyi) entropy. It uses a window to compute the information metric, which causes loss in time resolution, and thus early detection ability. 
In Fig. \ref{f:odit-mult}, it is seen that the cooperation among nodes facilitates earlier detection. Through the proposed computationally efficient cooperation scheme, given in Section \ref{s:coop}, the ODIT-based IDS is able to handle large networks with thousands of devices. This result can be easily extended to even larger networks with millions of devices. 
%}

The Receiver Operating Characteristic (ROC) curve for the mitigation performance is shown in Fig. \ref{f:mitigation}. It is clearly seen that the attacked devices are successfully identified with area under the curve (AUC) close to $1$, whereas the straightforward filtering method has a poor mitigation performance with AUC close the random guess value of $0.5$. The filtering method simply identifies a device as ``under attack" if its data rate exceeds a tolerable level. 

%The proposed IDS scales well to the networks with thousands of devices, as shown in Fig. \ref{f:odit1000}. It maintains its real-time operation and detects stealth DDoS attacks when only $5\%$ of the devices are attacked by means of $20\%$ increase in the packet rates. \tb{blah blah}

\begin{table}
\centering
\begin{tabular}{ |p{2cm}||p{1.3cm}|p{.8cm}||p{1.3cm}|p{.8cm}|  }

 \hline
 \multicolumn{5}{|c|}{Data Model} \\
 \hline
 \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ IoT~Devices & Active State Probability &  Mean Packet Rate &  Idle \ \ \ \ State Probability &  Mean Packet Rate\\
 \hline
Thermostat&	0.25&25&0.75&5\\
Smart Light&0.05&10&0.95&5\\
Security Camera&1&80&0&0\\
Smart Printer&0.05&75&0.95&5\\
Smart TV&0.3&120&0.7&10\\
\hline
\end{tabular}
\vspace{3mm}
\caption{Data Model representing different IoT devices and their Active state and Idle state probabilities.}
\label{table:2}
\vspace{-7mm}
\end{table}
